Satisfiability and Model Checking for the Logic of Sub-Intervals under the Homogeneity Assumption

The expressive power of interval temporal logics (ITLs) makes them one of the most natural choices in a number of application domains, ranging from the specification and verification of complex reactive systems to automated planning. However, for a long time, because of their high computational complexity, they were considered not suitable for practical purposes. The recent discovery of several computationally well-behaved ITLs has finally changed the scenario. In this paper, we investigate the finite satisfiability and model checking problems for the ITL D, that has a single modality for the sub-interval relation, under the homogeneity assumption (that constrains a proposition letter to hold over an interval if and only if it holds over all its points). We first prove that the satisfiability problem for D, over finite linear orders, is PSPACE-complete, and then we show that the same holds for its model checking problem, over finite Kripke structures. In such a way, we enrich the set of tractable interval temporal logics with a new meaningful representative.

==> D_SAT_hard.tex <==
\section{Hardness of satisfiability for \hsDhom{} over finite linear orders}\label{sec:SAThard}
In this section, we prove that the satisfiability problem for \hsDhom-formulas over finite linear orders is $\Psp$-hard. 
%
The construction mimics that of Sections 3.2 and 3.3 of \cite{DBLP:journals/fuin/MarcinkowskiM14}, Where the authors show that it is possible to build a formula $\Psi$ of \hsD{} which encodes accepting computations of an NFA. More precisely, the set of proposition letters of $\Psi$ is equal to the union of the alphabet of the NFA and the set of its states (plus some auxiliary letters, to enforce the \lq\lq orientation\rq\rq{} in the linear order, something that \hsD{} is unaware of), and $\Psi$ is satisfied by all and only the models such that the point-intervals are labeled with an accepting computation of the NFA over the word written in its point-intervals.

Then, $\Psi$ is exploited to encode the Kripke structure introduced in the previous section, thus getting a reduction from the problem of non-universality of the language recognized by an NFA to the satisfiability problem for \hsDhom.
As a matter of fact, a Kripke structure can be regarded as a trivial NFA over a unary alphabet, say $\{a\}$, such that all the states are final, as we are interested only in the structure of traces, that is, any word/trace is accepted under the only constraint that it exists in the structure.

By an easy adaptation of the results of Sections 3.2 and 3.3 of \cite{DBLP:journals/fuin/MarcinkowskiM14}, we obtain the~following proposition.
\begin{prop}\label{prop:MM}
    Let $\Ku=(\AP,\States, \Edges,\mu,\sinit)$ be a Kripke structure devoid of self-loops. Then, there exists a \hsDhom-formula $\Psi_{\Ku}$ whose set of proposition letters is $\AP\cup\States\cup Aux$---being $Aux$ a set of auxiliary letters---such that any finite linear order satisfying $\Psi_{\Ku}$ represents an initial trace of $\Ku$.
    Moreover, the size of $\Psi_{\Ku}$ is polynomial in the size of $\Ku$.
\end{prop}
Every linear order satisfying $\Psi_{\Ku}$ features states of $\Ku$ labeling point-intervals (exactly one state for each point).
Moreover, for each occurrence of some state $s$ of $\Ku$ along the order, we can easily force the set of letters $\mu(s)$ to hold on the same position (point).
The structure $\Ku$ in Proposition~\ref{prop:MM} must not feature self-loops for a technical reason: by fulfilling this requirement, there is no way for a state of $\Ku$ to \lq\lq span\rq\rq{} (by homogeneity) more than one point in a linear order satisfying $\Psi_{\Ku}$.
%
We observe that in~\cite{DBLP:journals/fuin/MarcinkowskiM14} the authors do not assume homogeneity; however, homogeneity does not cause any problem in our construction, as, intuitively, all the significant properties stated by $\Psi_{\Ku}$ are related to point-intervals.

Now, we observe that the Kripke structure of the previous section does not contain self-loops.
%
By Lemma~\ref{lemma:nuniv}, the language of an NFA $\mathcal{N}$ is non-universal if and only if there exists an initial trace $\rho$ such that $\Ku_\mathcal{N},\rho\models \Phi_\mathcal{N}$ (the Kripke structure and formula built from $\mathcal{N}$ in the previous section) if and only if (by Proposition~\ref{prop:MM} applied to $\Ku_\mathcal{N}$) the formula $\Psi_{\Ku_\mathcal{N}}\wedge\Phi_\mathcal{N}$ is satisfiable. This allows us to conclude that the following theorem holds (we also recall Theorem \ref{thm:pspace}).
%
\begin{thm}\label{cor:pspace_complete}
The satisfiability problem for \hsDhom-formulas over finite linear orders is $\Psp$-complete.
\end{thm} 

==> D_modelchecking_hard.tex <==
\section{Hardness of MC for \hsDhom{} over finite Kripke structures}\label{sec:MChard}
In this section, we prove %the
$\Psp$-hardness of MC for \hsDhom{} over finite Kripke structures
by means of a polynomial-time reduction from the $\Psp$-complete \emph{problem of (non-) universality} of the language of an NFA~\cite{holzer}.
We start by recalling some basic notions.


Let $\mathcal{N} =(\Sigma,Q,q_1,\delta,F)$ be an NFA over some alphabet $\Sigma$.
It is well-known that, by a subset construction, we can build a DFA $\tilde{\mathcal{N}} =(\Sigma,\tilde{Q},\tilde{q_1},\tilde{\delta},\tilde{F})$  such that $\mathcal{L}(\tilde{\mathcal{N}})=\mathcal{L}(\mathcal{N})$ and~$\tilde{Q}= 2^{Q}$.
The problem of deciding whether $\mathcal{L}(\mathcal{N})\neq\emptyset$ for an NFA $\mathcal{N}$ can be solved with \emph{logarithmic working space} by means of a nondeterministic reachability test from the initial state of $\mathcal{N}$ to an accepting state. On the other hand, establishing whether $\mathcal{L}(\mathcal{N})$ is \emph{non-universal}, that is, $\mathcal{L}(\mathcal{N})\neq\Sigma^*$, which amounts to check whether there is $w\in\Sigma^*$ such that $w\notin\mathcal{L}(\mathcal{N})$,  is a $\Psp$-complete problem~\cite{holzer}. This is because the length of the shortest word \emph{not accepted} by an NFA may be exponential in the number of its states.

To check whether a word $w$ is accepted by an NFA $\mathcal{N}$, one can build \lq\lq on the fly\rq\rq{} the computation of the equivalent DFA $\tilde{\mathcal{N}}$
%(with $\mathcal{L}(\tilde{\mathcal{N}})=\mathcal{L}(\mathcal{N})$),
(obtained from $\mathcal{N}$ by the subset construction) over $w$.

\begin{figure}[t]
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick]
  %\tikzstyle{every state}=[fill=red,draw=none,text=white]

  \node[initial,state] (A)              {$q_1$};
  \node[state]         (B) [right of=A] {$q_2$};
  \node[state,accepting](C)[right of=B] {$q_3$};

  \path (A) edge              node {$a$} (B)
        (B) edge [bend right] node {$a$} (C)
        (B) edge [loop above] node {$c$} (B)
        (B) edge [bend left] node {$b$} (C)
        (A) edge [loop above] node {$a$} (A)
        (A) edge [loop below] node {$b$} (A);
    \end{tikzpicture}
    \caption{An NFA with initial state $q_1$ and final state $q_3$.}\label{fig:Nfa}
\end{figure}
Let $\mathcal{N}$ be the NFA of Figure \ref{fig:Nfa}. The computation of the equivalent DFA $\tilde{\mathcal{N}}$ on $aab$ is:
\begin{equation}
    (Q_1=\{q_1\}) \stackrel{a}{\to}
    (Q_2=\{q_1,q_2\}) \stackrel{a}{\to}
    (Q_3=\{q_1,q_2,q_3\}) \stackrel{b}{\to} (Q_4=\{q_1,q_3\}),
\label{eq:1}\end{equation}
where $Q_1$ is the initial state of $\tilde{\mathcal{N}}$. Since $Q_4$ (the state of $\tilde{\mathcal{N}}$ reached by the computation) contains the final state $q_3$ of $\mathcal{N}$, $aab$ is accepted.
%
The computation of $\tilde{\mathcal{N}}$ on $aac$ is:
\begin{equation}
    (Q_1=\{q_1\}) \stackrel{a}{\to}
    (Q_2=\{q_1,q_2\}) \stackrel{a}{\to}
    (Q_3=\{q_1,q_2,q_3\}) \stackrel{c}{\to} (Q_4'=\{q_2\})
\end{equation}
Since $Q_4'$ does not contain the final state of $\mathcal{N}$, $aac$ is \emph{not} accepted.

As a general rule, given a word $w$, with $|w|=n$, in the computation of $\tilde{\mathcal{N}}$ on $w$
\[
    Q_1 \stackrel{w[0])}{\to}
    Q_2 \stackrel{w[1]}{\to}
    \cdots \stackrel{w[n-2]}{\to}
    Q_{n} \stackrel{w[n-1]}{\to} Q_{n+1},
\]
the state $q$ of $\mathcal{N}$ is in $Q_i$, for $0\leq i\leq n$, \emph{if and only if} there is a computation of $\mathcal{N}$ on $w$
\[  q_1 \stackrel{w[0]}{\to}
    q_2 \stackrel{w[1]}{\to}
    \cdots \stackrel{w[n-2]}{\to}
    q_{n} \stackrel{w[n-1]}{\to} q_{n+1}
\]
where $q=q_i$.
Moreover, if some $q\in Q_{i}$, then all $q'\in\delta(q,w[i-1])$ must be in $Q_{i+1}$ ($\delta$ is the transition function of the NFA $\mathcal{N}$). Conversely, if some $q'\in Q_{i+1}$, then there must be some $q\in Q_i$ such that $q'\in\delta(q,w[i-1])$.

We are now ready to provide a polynomial-time reduction of the $\Psp$-complete problem of (non-)universality of the language of an NFA to the MC problem for \hsDhom{} over finite Kripke structures. %
%, proving that the latter is $\Psp$-hard.

Let $\mathcal{N} =(\Sigma,Q,q_1,\delta,F)$, with $Q=\{q_1,\ldots,q_{|Q|}\}$, be an NFA. We build a Kripke structure $\Ku_\mathcal{N}$ and a \hsDhom{} formula $\Phi_\mathcal{N}$ such that there is a computation of the DFA $\tilde{\mathcal{N}}$ which is not accepting if and only if there is an initial  trace $\rho$ of $\Ku_\mathcal{N}$ which satisfies $\Phi_\mathcal{N}$. Hence, the language accepted by $\mathcal{N}$ is universal if and only if $\Ku_\mathcal{N} \models \neg\Phi_\mathcal{N}$. Intuitively, the computations of $\tilde{\mathcal{N}}$ are encoded by suitable initial traces of $\Ku_\mathcal{N}$, while $\Phi_\mathcal{N}$ captures all and only those initial traces of $\Ku_\mathcal{N}$ which encode non-accepting computations of $\tilde{\mathcal{N}}$.

We define the Kripke structure $\Ku_\mathcal{N}$ as the tuple $(\AP,\States, \Edges,\mu,\sinit)$, where:
\begin{itemize}
    \item $\AP=\{q_i,q_i'\mid i=1,\ldots, |Q|\}\cup\Sigma\cup\{e_1,e_2,f_1,f_2\}$;
    \item $\States=\{q_i^\top,q_i^\bot,q_i'^\top,q_i'^\bot\mid i=1,\ldots, |Q|\}\cup\{x_1,x_2,v_1,v_2,v'_1,v'_2, \widehat{q_1}^\top,\widehat{q_2}^\bot, \ldots,\widehat{q_{|Q|}}^\bot\}\cup\Sigma$;
    \item $\sinit=v_1'$;
    \item the labeling function $\mu$ is defined as follows:
    \begin{itemize}
      \item     $\mu({q_i}^\top)=\mu({q_i'}^\top)=\AP$, $\mu({q_i}^\bot)=\AP\setminus\{q_i\}$, $\mu({q'_i}^\bot)=\AP\setminus\{q_i'\}$, for $1\leq i\leq |Q|$;
    \item $\mu(a)=\AP\setminus(\Sigma\setminus\{a\})$, for $a\in\Sigma$;
   \item  $\mu(x_1)=\AP\setminus\{e_1\}$,  $\mu(x_2)=\AP\setminus\{e_2\}$;
   \item  $\mu(v_1)=\mu(v_1')=\AP\setminus\{f_1\}$,
    $\mu(v_2)=\mu(v_2')=\AP\setminus\{f_2\}$;
    \item $\mu(\widehat{q_1}^\top)=\AP$,
    $\mu(\widehat{q_2}^\bot)=\AP\setminus\{q_2\}$, $\mu(\widehat{q_3}^\bot)=\AP\setminus\{q_3\}$, \dots , $\mu(\widehat{q_{|Q|}}^\bot)=\AP\setminus\{q_{|Q|}\}$.
    \end{itemize}
\end{itemize}

%Without loss of generality,
The set of edges $\Edges$ for an arbitrary NFA can be easily deduced  from Figure~\ref{fig:HardKu}, where the Kripke structure built for an NFA with $Q=\{q_1,q_2,q_3\}$ and $\Sigma = \{a,b,c\}$ is depicted.
%
\begin{figure}[t]
    \centering
    \resizebox{\textwidth}{!}{\input{HardKripke}}
    %\vspace*{-0.7cm}
    \caption{The Kripke structure $\Ku_\mathcal{N}$ for an NFA with $Q=\{q_1,q_2,q_3\}$ and  $\Sigma=\{a,b,c\}$.}
    \label{fig:HardKu}
\end{figure}
%
The idea is to encode the computation of $\tilde{\mathcal{N}}$ on a given word by an initial trace. As an example, the computation of $\tilde{\mathcal{N}}$ on $aab$, described in Equation~\ref{eq:1},
is represented by the following initial trace of $\Ku_\mathcal{N}$:
\begin{equation}\begin{split}
v_1'v_2'\underbrace{(\widehat{q_1}^\top\widehat{q_2}^\bot\widehat{q_3}^\bot)}_{Q_1} a x_1x_2 \underbrace{({q'_1}^\top {q'_2}^\top {q'_3}^\bot)}_{Q'_2}\cdots\\
v_1v_2 \underbrace{({q_1}^\top {q_2}^\top {q_3}^\bot)}_{Q_2} a x_1x_2 \underbrace{({q'_1}^\top {q'_2}^\top {q'_3}^\top)}_{Q'_3} \cdots\\
v_1v_2 \underbrace{({q_1}^\top {q_2}^\top {q_3}^\top)}_{Q_3} b x_1x_2 \underbrace{({q'_1}^\top {q'_2}^\bot {q'_3}^\top)}_{Q'_4} \cdots\\
v_1v_2 \underbrace{({q_1}^\top {q_2}^\bot {q_3}^\top)}_{Q_4}.
\end{split}
\label{eq:extrack}
\end{equation}

The states $v_1,v'_1,v_2,v'_2,x_1$, and $x_2$ are introduce for technical reasons, that will be explained later.
%
A triple of states $({q_1}^* {q_2}^* {q_3}^*)$, where $^*$ stands for $\top$ or $\bot$, represents the state $Q_i$ of $\tilde{\mathcal{N}}$ reached at the $(i-1)$-th step of the computation before reading $w[i-1]$: we have ${q_j}^\top$ if $q_j\in Q_i$ and ${q_j}^\bot$ if $q_j\not\in Q_i$.
Hereafter, we denote each triple $({q_1}^* {q_2}^* {q_3}^*)$ by the corresponding $Q_i$.
Sub-traces denoted by $Q_i$ and $Q'_i$ must be copies, that is, ${q_j}^\top\in Q_i$ if and only if ${q'_j}^\top\in Q'_i$. In between $Q_i$ and $Q'_{i+1}$, the trace features the occurrence of $w[i-1]\in\Sigma$.
The states $\widehat{q_1}^\top$, $\widehat{q_2}^\bot$, and $\widehat{q_3}^\bot$ of $\Ku_\mathcal{N}$ are just \lq\lq copies\rq\rq{} of ${q_1}^\top$, ${q_2}^\bot$, and ${q_3}^\bot$, respectively, which are introduced to force the first state of the DFA $\tilde{\mathcal{N}}$ to be $Q_1=\{q_1\}$ (represented by $\widehat{q_1}^\top \widehat{q_2}^\bot \widehat{q_3}^\bot$).
Last but not least, there is a match between the sub-traces and the proposition letters that they satisfy. As an example, it holds that:
\[
    \Ku_\mathcal{N}, v_1v_2 ({q_1}^\top {q_2}^\top {q_3}^\top) b x_1x_2 ({q'_1}^\top {q'_2}^\bot {q'_3}^\top)\models
    (q_1\wedge q_2\wedge q_3)\wedge (q'_1\wedge\neg q'_2\wedge q'_3)\wedge (\neg a \wedge b \wedge \neg c).
\]

Let us  consider now the formula $\Phi_\mathcal{N}$.
%, built from $\mathcal{N}$.
We assume the \emph{strict} semantics of \hsDhom{}.

To begin with, we define the following formulas, which exploit the auxiliary states $v_1,v'_1,v_2,v'_2,x_1,$ and $x_2$ to ``select'' some suitable traces:
\[
    \varphi_{trans}=\neg f_1\wedge \neg f_2 \wedge \bD(f_1\wedge f_2) \wedge \D\top ,
\]
\[
    \varphi_{copy}= \neg e_2\wedge \neg e_1 \wedge \bD(e_1\wedge e_2) \wedge \D\top .
\]
% \[
%     \varphi'_{trans}=\neg e_2\wedge e_1 \wedge \neg f_1\wedge \neg f_2 ,
% \]
%
By construction, the following statements hold: %We can prove that:
\begin{itemize}
    \item $\Ku_\mathcal{N},\rho\models\varphi_{trans}$ if and only if $\rho=\tilde{v_2}\cdots v_1$,  where $\tilde{v_2}$ can be either $v_2$ or $v'_2$, and $v_1,v_2$ do not occur as internal states of $\rho$;
%    \item \textbf{$\Ku_\mathcal{N},\rho\models\varphi'_{trans}$ iff ($\rho=x_2\cdots v_1 v_2 q_1^*\cdots q_j^*$ for $j\geq 0$, or $\rho=x_2\cdots v_1 v_2 q_1^*\cdots q_{|Q|}^*c$ for some $c\in\Sigma$) and there are no occurrences of $x_1$ in $\rho$;}
    \item $\Ku_\mathcal{N},\rho\models\varphi_{copy}$ if and only if $\rho=x_2\cdots x_1$ and $x_1,x_2$ do not occur as internal states of $\rho$.
\end{itemize}

Moreover, we define the following pair of formulas, whose intended meaning is quite evident (in particular, $length_{\geq 3}$ is satisfied by a trace $\rho$ if and only if $|\rho|\geq 3$):
\[
    \varphi_{reject}= \bigwedge_{q_i\in F}\neg q_i, \mbox{ and }  length_{\geq 3}=\D\top .
\]
% \[
%     length_{\leq|Q|+2}=\underbrace{\bD\cdots\bD}_{\lceil\frac{|Q|}{2}\rceil+1\text{ times}} \bot ,
% \]
%\[
 %   length_{\geq 3}=\D\top .
%\]

The formula $\Phi_\mathcal{N}$ is defined as follows (for the sake of brevity, for $q_i,q_j\in Q$ and $c\in\Sigma$, we write $(q_i,c,q_j) \in \delta$ for $q_j\in\delta(q_i,c)$):
\begin{multline*}
    \Phi_\mathcal{N}:=
     \underbrace{\bD\Big(\varphi_{trans}\rightarrow \Big(\big(\bigwedge_{(q_i,a,q'_j)\in\delta}((q_i\wedge a)\rightarrow q'_j)\big) \wedge \big(\bigwedge_{q'_i\in Q} (q'_i\rightarrow \bigvee_{(q_j,a,q'_i)\in\delta} (q_j\wedge a))\big) \Big)\Big)}_{(1)}\wedge\\
     \underbrace{\bD\big( \varphi_{copy} \rightarrow \bigwedge_{q_i\in Q} (q_i\leftrightarrow q'_i) \big)}_{(2)}\wedge \underbrace{\Big((e_1\wedge length_{\geq 3}\wedge \varphi_{reject})\vee \D\Big(\varphi_{copy}\wedge\varphi_{reject}\Big)\Big)}_{(3)}
\end{multline*}

%For the sake of simplicity, in the following we assume w.l.o.g.\ that $\mathcal{N}$ has an even number of states (we may always add a non-final disconnected fresh state).
The next lemma proves that the construction is correct. %Let us now prove the following lemma.
\begin{lem}\label{lemma:nuniv}
Let $\mathcal{N}$ be an NFA. It holds that $\mathcal{L}(\mathcal{N})\neq \Sigma^*$ if and only if there exists an initial trace $\rho$ of $\Ku_\mathcal{N}$ such that $\Ku_\mathcal{N},\rho\models \Phi_\mathcal{N}$.
\end{lem}
%
\begin{proof}
$(\Rightarrow)$ If $\mathcal{L}(\mathcal{N})\neq \Sigma^*$, then there exists $w\notin\mathcal{L}(\mathcal{N})$. Thus, the computation of $\tilde{\mathcal{N}}$ over $w$ is \emph{not} accepting. Let $\rho$ be the initial trace of $\Ku_\mathcal{N}$ encoding such a computation (see Equation~\ref{eq:extrack} for an account of its structure).

We distinguish two cases:
\begin{itemize}
    \item $w=\varepsilon$:  we consider $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot\cdots \widehat{q_{|Q|}}^\bot $. No strict sub-trace satisfies $\varphi_{trans}$ or $\varphi_{copy}$, and hence conjuncts (1) and (2) are trivially satisfied. Moreover, since $\varepsilon\notin\mathcal{L}(\mathcal{N})$, $q_1\notin F$, and thus $\rho$ models also $e_1\wedge length_{\geq 3}\wedge \varphi_{reject}$.
    \item $w\neq \varepsilon$: we consider the initial trace $\rho$ of $\Ku_\mathcal{N}$ that encodes the computation on $w$, w.l.o.g.\ extended with some $c\in\Sigma$ (any symbol is fine), and finally $x_1 x_2$. Its generic form is $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot\cdots \widehat{q_{|Q|}}^\bot w[0](x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1x_2$, where $^*$ is $^\bot$ or $^\top$, and $^+$ denotes one or more occurrences of the string in brackets. Every strict sub-trace satisfying $\varphi_{trans}$ models the right part of the implication in conjunct (1), which enforces the consistency conditions of a computation.
    Every strict sub-trace satisfying $\varphi_{copy}$ features ${q'_i}^\top$ if it features ${q_i}^\top$, and ${q'_i}^\bot$ if it features ${q_i}^\bot$, and hence satisfies $\bigwedge_{q_i\in Q} (q_i\leftrightarrow q'_i)$. Finally, the last part of $\rho$, namely, $x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c x_1$,
    models $\varphi_{copy}$, and since $w$ is \emph{not} accepted, it also fulfills $\varphi_{reject}$.
\end{itemize}
This allows us to conclude that, in both cases, there exists an initial trace $\rho$ such that $\Ku_\mathcal{N},\rho\models \Phi_\mathcal{N}$.

$(\Leftarrow)$ Let us assume that there exists an initial trace $\rho$ of $\Ku_\mathcal{N}$ such that $\Ku_\mathcal{N},\rho\models \Phi_\mathcal{N}$. We distinguish a number of cases, according to the structure of $\rho$.
\begin{enumerate}
    \item $\rho=v'_1(v'_2)^?$ ($^?$ denotes 0 or 1 occurrences of the string in brackets).
    This trace does not satisfy (3), thus it cannot be the trace we are looking for.
    %
    \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_j}^\bot$, for $j\geq 1$, or $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c$, for some $c\in\Sigma$.
    No sub-trace satisfies $\varphi_{copy}$, thus, by (3), $\rho$ satisfies $\varphi_{reject}$. Hence, $q_1\notin F$, and $\varepsilon$ is rejected by $\mathcal{N}$.
    %
    \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c x_1(x_2)^?$.
    This trace does not satisfy (3).
    %
    \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_j}^*$, for $j\geq 1$.
    This trace does not satisfy (3).
    %
    \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1(v_2)^?$.
    This trace does not satisfy (3).
    %
    \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_j}^*$.
    This trace does not satisfy (3).
    %
    \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c$.
    This trace does not satisfy (3).
    %
   % \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*cx_1$\\
   % This trace does not model the conjunct (3).
    %
    \item\label{case:A} $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c (x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1(x_2)^{?}$.
    Since $\rho$ satisfies (1), \emph{all} adjacent pairs of occurrences of ${q_1}^*{q_2}^*\cdots {q_{|Q|}}^*\rightsquigarrow{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*$ consistently model a transition of $\tilde{\mathcal{N}}$; moreover, \emph{all} adjacent pairs of occurrences of ${q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*\rightsquigarrow {q_1}^*{q_2}^*\cdots {q_{|Q|}}^*$ are ``copies''. Therefore, a legal computation of $\tilde{\mathcal{N}}$ on some string $w$ is encoded. Finally, by (3), a strict sub-trace $x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c x_1$ satisfies $\varphi_{reject}$. Thus, either $w$ (if such a sub-trace is the last one) or one of its prefixes (if it is not the last one) is rejected by $\tilde{\mathcal{N}}$.
    %
    \item\label{case:B} $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c (x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1x_2\underline{{q'_1}^*{q'_2}^*\cdots {q'_j}^*}$.
    In this case, as well as in the following ones, we underline the final part of $\rho$ which may be ``garbage'', that is, it may encode an illegal suffix of a computation, just because it is not forced to ``behave correctly'' by $\Phi_\mathcal{N}$.
    However, since (3) is satisfied, a strict sub-trace $x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c x_1$ satisfies $\varphi_{reject}$ (and this is not part of the garbage). Thus, as before, some word $w$ or one of its prefixes is rejected by $\tilde{\mathcal{N}}$.
    %
    \item $\rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c (x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1x_2\underline{{q'_1}^*{q'_2}^*\!\cdots {q'_{|Q|}}^*v_1}$.
    Like the previous case.
    %
    \item\label{case:C} The next case can be dealt with as case~(\ref{case:A}), but a prefix of $w$ is necessarily rejected, so that $\rho$ encodes the computation of $\tilde{\mathcal{N}}$ on $w$:
    \[\begin{split}
    \rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c (x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1\cdot \\
    x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2.
    \end{split}\]
    %
    \item All the following cases can be dealt with as case~(\ref{case:C}), just with the addition of final garbage, which is not considered, since it is not part of a strict sub-trace satisfying $\varphi_{copy}$:
        \[\begin{split}
        \rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c (x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1\cdot \\
        x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2\underline{{q_1}^*{q_2}^*\cdots {q_j}^*};
        \end{split}\]
        %
        \[\begin{split}
        \rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c (x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1\cdot \\
        x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2\underline{{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c};
        \end{split}\]
        %
        \[\begin{split}
        \rho=v'_1v'_2\widehat{q_1}^\top\widehat{q_2}^\bot \cdots \widehat{q_{|Q|}}^\bot c (x_1x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c)^+x_1\cdot \\
        x_2{q'_1}^*{q'_2}^*\cdots {q'_{|Q|}}^*v_1v_2\underline{{q_1}^*{q_2}^*\cdots {q_{|Q|}}^*c x_1}.
        \end{split}\]
\end{enumerate}
Since in all possible (legal) cases we get that some string is rejected by $\tilde{\mathcal{N}}$ (and thus by $\mathcal{N}$), the thesis immediately follows.
\end{proof}

By Lemma~\ref{lemma:nuniv}, we have that $\mathcal{L}(\mathcal{N})= \Sigma^*$ if and only if $\Ku_\mathcal{N}\models \neg\Phi_\mathcal{N}$. Since the \emph{problem of universality} of the language recognized by an NFA is $\Psp$-complete, % (because $\Psp$ is closed under complement),
and both $\Ku_\mathcal{N}$ and $\Phi_\mathcal{N}$ can be generated in polynomial time, taking into account the upper bound given by Theorem~\ref{thm:pspaceMC}, we have proved the main result of the section.

\begin{thm}
The MC problem for \hsDhom-formulas over finite Kripke structures is \mbox{$\Psp$-complete}.
\end{thm}

In addition, we can state the following theorem.

\begin{thm}
The MC problem for \emph{constant-length} \hsDhom-formulas over finite Kripke structures is $\NLOGSP$-complete.
\end{thm}
\begin{proof}
Membership is given by Theorem~\ref{thm:pspaceMC}.
As for $\NLOGSP$-hardness, there is a trivial reduction from the \emph{problem of \mbox{(non-)reachability}} of two nodes in a directed~graph.
\end{proof}

By slightly modifying $\Phi_\mathcal{N}$, we can adapt the proof to \hsDhom{} with the \emph{proper} semantics.
In the next section, we will come back to satisfiability, and prove that it is a $\Psp$-complete problem as well. 


%%%%%%%%%%%%%%%%%
\begin{enumerate}
  \item \emph{Propositional mutual exclusion}: at every position, at most one proposition holds. This can be expressed in
  \hsDhom{} by the formula
  %
  \[
\neg \displaystyle{\bigvee_{p,p'\in\AP\mid p\neq p'} \D (p\wedge p')
  \]
  %
  \item \emph{Initialization}: there is some position where $(d_\Init,0,b)$ holds for some color $b\in\{0,1\}$. This is captured by the
  formula
  %
    \[
     \displaystyle{\bigvee_{b\in\{0,1\}}} \D  (d_\Init,0,b)
    \]
    %
  \item \emph{$n$-length constraint}: there is some infix of the given word $w$ ($w$ included) having length
  $n$ and such that all its positions have the same color. This requirement can be formalized in \hsDhom{} as
     %
    \[
    \D \psi \wedge \psi\quad\quad\text{where }\psi:= len_{=n} \wedge displaystyle{\bigvee_{b\in \{0,1\}}} \bD (len_{=1} \rightarrow  displaystyle{\bigvee_{d\in \Delta}\bigvee_{i\in [1,n]}})
    \]
    %
\end{enumerate}
